Soft and Jet functions for SCET at four loops in QCD

Soft-Collinear Effective Theory is a framework for systematically organizing and resumming the logarithmic contributions that occur in high-energy reactions. It provides a factorized description of cross sections in terms of hard, jet, soft, and beam functions. As the latter are universal, they can be obtained from the well-known perturbative results in quantum chromodynamics (QCD) for deep-inelastic scattering, Drell-Yan and Higgs boson productions. Using the recent results ~\cite{Kniehl:2025ttz} on four-loop eikonal $(f^I)$ and collinear anomalous dimensions $(B^I)$ for quarks and gluons, $I=q,g$, as well as perturbative results from previous orders, we present four-loop predictions for the quark and gluon soft and jet functions. They constitute an important component of the $N$-jettiness subtraction method at $\rm{N^4LO}$ accuracy in QCD, which eventually may enable the calculation of fully-differential cross sections at higher orders.

==> ChiDYg.tex <==
\begin{align}
   \chi^{g}_{{\rm S},1} &=
        C_A   \bigg\{  - 3 \zeta_2 \bigg\}\,, 
\nonumber\\
   \chi^{g}_{{\rm S},2} &=
        C_A^2   \bigg\{ \frac{2428}{81} - \frac{374}{9} \zeta_3 - \frac{469}{9} \zeta_2 + 4 \zeta_2^2 \bigg\}
       - C_A n_f   \bigg\{   \frac{328}{81} - \frac{68}{9} \zeta_3 - \frac{70}{9} \zeta_2 \bigg\}\,, 
\nonumber\\
   \chi^{g}_{{\rm S},3} &=
        C_A^3   \bigg\{ \frac{5211949}{8748} - \frac{484}{3} \zeta_5 - \frac{128966}{81} \zeta_3 + \frac{536}{3} \zeta_3^2
          - \frac{578479}{486} \zeta_2 + 726 \zeta_2 \zeta_3 + \frac{9457}{45} \zeta_2^2 + \frac{152}{63}
         \zeta_2^3 \bigg\}
\nonumber\\&         
       - C_A^2 n_f   \bigg\{   \frac{412765}{4374} + 8 \zeta_5 - \frac{9856}{27} \zeta_3 - \frac{75155}{243}
         \zeta_2 + 44 \zeta_2 \zeta_3 + \frac{2528}{45} \zeta_2^2 \bigg\}
       - C_A n_f^2   \bigg\{   \frac{128}{2187} + \frac{1480}{81} \zeta_3 + \frac{404}{27} \zeta_2 - \frac{148}{45}
         \zeta_2^2 \bigg\}
\nonumber\\&         
       - C_F C_A n_f   \bigg\{   \frac{42727}{324} - \frac{112}{3} \zeta_5 - \frac{2284}{27} \zeta_3 - \frac{605}{6} \zeta_2
          + 88 \zeta_2 \zeta_3 - \frac{152}{15} \zeta_2^2 \bigg\}
\end{align}
